Gradient Free Minimax Optimization: Variance Reduction and Faster Convergence

Many important machine learning applications amount to solving minimax optimization problems, and in many cases there is no access to the gradient information, but only the function values. In this paper, we focus on such a gradient-free setting, and consider the nonconvex-strongly-concave minimax stochastic optimization problem. In the literature, various zeroth-order (i.e., gradient-free) minimax methods have been proposed, but none of them achieve the potentially feasible computational complexity of $\mathcal{O}(\epsilon^{-3})$ suggested by the stochastic nonconvex minimization theorem. In this paper, we adopt the variance reduction technique to design a novel zeroth-order variance reduced gradient descent ascent (ZO-VRGDA) algorithm. We show that the ZO-VRGDA algorithm achieves the best known query complexity of $\mathcal{O}(\kappa(d_1 + d_2)\epsilon^{-3})$, which outperforms all previous complexity bound by orders of magnitude, where $d_1$ and $d_2$ denote the dimensions of the optimization variables and $\kappa$ denotes the condition number. In particular, with a new analysis technique that we develop, our result does not rely on a diminishing or accuracy-dependent stepsize usually required in the existing methods. To our best knowledge, this is the first study of zeroth-order minimax optimization with variance reduction. Experimental results on the black-box distributional robust optimization problem demonstrates the advantageous performance of our new algorithm.

==> preliminaries.tex <==


\subsection{Notation and Preliminaries}

In this paper, we use $\ltwo{\cdot}$ to denote the Euclidean norm of vectors. For a finite set $\mathcal{S}$, we denote its cardinality as $\lone{\mathcal{S}}$. For a positive integer $n$, we denote $[n]=\{1,\cdots,n\}$. We assume that the min-max problem \cref{eq: 2} satisfies the following assumptions, which have also been adopted by \cite{luo2020stochastic} for SREDA. We slightly abuse the notation $\xi$ below to represent the random index in both the online and finite-sum cases, where in the finite-sum case, $\mE_{\xi}[\cdot]$ is with respect to the uniform distribution over $\{\xi_1,\cdots,\xi_n\}$. 

\begin{assumption}\label{ass1}
	The function $\Phi(\cdot)$ is lower bounded, i.e., we have $\Phi^*=\inf_{x\in \mR^{d_1}}\Phi(x) > -\infty$.
\end{assumption}
%%%
\begin{assumption}\label{ass2}
	The component function $F$ has an averaged $\ell$-Lipschitz gradient, i.e., for all $(x,y)$, $(x^\prime,y^\prime)\in \mR^{d_1}\times \mR^{d_2}$, we have $\mE_\xi\big[\ltwo{\nabla F(x,y;\xi)-\nabla F(x^\prime,y^\prime;\xi)}^2\big]\leq \ell^2(\ltwo{x-x^\prime}^2+\ltwo{y-y^\prime}^2)$.
%	\begin{flalign*}
%		\mE_\xi\big[\ltwo{\nabla F(x,y;\xi)-\nabla F(x^\prime,y^\prime;\xi)}^2\big]\leq \ell^2(\ltwo{x-x^\prime}^2+\ltwo{y-y^\prime}^2).
%	\end{flalign*}
\end{assumption}
%\textcolor{red}{[Is the above assumption applicable only for online case? If so, what about finite-sum case?]}

%%%%%%%%%%%%%%%%%%%%
%We further take the following assumption, which was also adopted in \cite{luo2020stochastic} for the analysis of SREDA.
\begin{assumption}\label{ass3}
	The function $f$ is $\mu$-strongly-concave in $y$ for any $x\in\mR^{d_1}$, and the component function $F$ is concave in $y$, i.e., for any $x\in \mR^{d_1}$, $y,y^\prime\in \mR^{d_2}$ and $\xi$, we have $f(x,y)\leq f(x,y^\prime) + \langle \nabla_y f(x,y^\prime), y-y^\prime \rangle - \frac{\mu}{2}\ltwo{y-y^\prime}$, and $F(x,y;\xi)\leq F(x,y^\prime;\xi) + \big\langle \nabla_y F(x,y^\prime;\xi), y-y^\prime \big\rangle$.
%	\begin{flalign*}
%	f(x,y)\leq f(x,y^\prime) + \langle \nabla_y f(x,y^\prime), y-y^\prime \rangle - \frac{\mu}{2}\ltwo{y-y^\prime},
%	\end{flalign*}
%	and
%	\begin{flalign*}
%	F(x,y;\xi)\leq F(x,y^\prime;\xi) + \big\langle \nabla_y F(x,y^\prime;\xi), y-y^\prime \big\rangle.
%	\end{flalign*}
\end{assumption}
%\textcolor{red}{[should the above assumption holds for all $\xi$ with the same $\mu$?]}

%%%%%%%%%%%%%%%%%%%%%
%\edef\oldassumption{\the\numexpr\value{assumption}+1}
%\setcounter{assumption}{0}
%\renewcommand{\theassumption}{\oldassumption.\alph{assumption}}
%\begin{assumption}\label{ass6}
%	he component function $F$ is $\mu$-strongly-concave in $y$, i.e., there exists a constant $\mu>0$ such that for any $x\in \mR^{d_1}$ and $y,y^\prime\in \mR^{d_2}$, we have
%	\begin{flalign*}
%	F(x,y,\xi)\leq F(x,y^\prime,\xi) + \big\langle \nabla_y F(x,y^\prime,\xi),y-y^\prime \big\rangle - \frac{\mu}{2}\ltwo{y-y^\prime}^2.
%	\end{flalign*}
%\end{assumption}
%%%%%%%%%%%%%%%%%%%%
%\begin{assumption}\label{ass3}
%	The function $f$ is $\mu$-strongly-concave in $y$ for any $x\in\mR^{d_1}$, and the component function $F$ is concave in $y$, i.e., for any $x\in \mR^{d_1}$, $y,y^\prime\in \mR^{d_2}$ and random vector $\xi$, we have
%	\begin{flalign*}
%	F(x,y;\xi)\leq F(x,y^\prime;\xi) + \big\langle \nabla_y F(x,y^\prime;\xi), y-y^\prime \big\rangle.
%	\end{flalign*}
%\end{assumption}
%\let\theassumption\origtheassumption
%%%%%%%%%%%%%%%%%%%%
%%%
%\addtocounter{assumption}{+1}
%%%
\begin{assumption}\label{ass5}
	The gradient of each component function $F(x,y;\xi)$ has a bounded variance, i.e., there exists a constant $\sigma>0$ such that for any $(x,y)\in \mR^{d_1 \times d_2}$, we have $\mE_\xi\big[\ltwo{\nabla F(x,y;\xi)-\nabla f(x,y)}^2\big]\leq \sigma^2<\infty$.
%	\begin{flalign*}
%		\mE_\xi\big[\ltwo{\nabla F(x,y;\xi)-\nabla f(x,y)}^2\big]\leq \sigma^2<\infty.
%	\end{flalign*}
\end{assumption}
%\textcolor{red}{[Is the above assumption applicable only for online case? If so, what about finite-sum case?]}

%\textcolor{red}{[Is the above assumption also taken by SREDA?]}
%%%
%The gradient-Lipschitz assumption is standard in the optimization literature, stronlgy concavity is crucial here, allowing for an efficient solution of $\max_{y\in \mR^{d_2}}f(x,\cdot)$. 

%We define $\kappa\triangleq\ell/\mu$ as the condition number of the problem throughout the paper. The following structural lemma developed in \cite{lin2019gradient} provides further information about $\Phi$ for nonconvex-strongly-concave min-max optimization.
%\begin{lemma}[Lemma 3.3 of \cite{lin2019gradient}]\label{lemma1}
%	Under \Cref{ass2} and \Cref{ass6}, the function $\Phi(\cdot)=\max_{y\in \mR^{d_2}}f(\cdot,y)$ is $(\kappa+1)\ell$-gradient Lipschitz and $\nabla \Phi(x)=\nabla_x f(x, y^*(x))$ is $\kappa$-Lipschitz, where $y^*(\cdot)=\argmin_{y\in\mR^{d_2}}f(\cdot,y)$.
%\end{lemma}
%We let $L\triangleq (1+\kappa)\ell$ denote the Lipschitz constant of $\nabla\Phi(x)$. 
Since $\Phi$ is nonconvex in general, it is NP-hard to find its global minimum. The goal here is to develop stochastic gradient algorithms that output an $\epsilon$-stationary point as defined below.
\begin{definition}
	The point $\bar{x}$ is called an $\epsilon$-stationary point of the differentiable function $\Phi$ if $\ltwo{\nabla \Phi(\bar{x})}\leq \epsilon$, where $\epsilon$ is a positive constant.
\end{definition}

